Functoriality for the su(3) Khovanov homology

We prove that Morrison and Nieh's categorification of the su(3) quantum knot invariant is functorial with respect to tangle cobordisms. This is in contrast to the categorified su(2) theory, which was not functorial as originally defined. We use methods of Bar-Natan to construct explicit chain maps for each variation of the third Reidemeister move. Then, to show functoriality, we modify arguments used by Clark, Morrison, and Walker to show that induced chain maps are invariant under Carter and Saito's movie moves.

==> sections/background_thesis.tex <==
\section{
Background}
\label{sec:background}

In 1984 Jones discovered his famous polynomial invariant of links in the three-sphere and inaugurated the field of quantum topology. Interest was wide-spread. Algebraists, for example, saw a novel application of subfactors of von Neumann algebras and would soon embark upon the study of quantum groups, while physicists noticed connections with statistical mechanics and quantum field theory. Topologists, on the other hand, recognized a link invariant of unexpected power. Even more exciting was the fact that the Jones polynomial admitted a very simple combinatorial definition \cite{Kauf87_MR899057}, making it highly computable. Proofs of the long-standing Tait conjectures for alternating knots followed shortly thereafter \cite{Mur87_MR895570}, as did this extension: for any simple Lie algebra $\mathfrak{g}$, there is a quantum group $U_q (\mathfrak{g})$ and a link invariant that is a polynomial in $q$; this extends to a three-manifold invariant for $q$ a root of unity \cite{Ohts96_MR1374199}.

For all the computational power these new tools provided, however, they lacked the transparency of classical invariants like the Alexander polynomial or Arf invariant. Classical invariants, on the one hand, are geometrically grounded in the objects they are trying to study. Applying and interpreting them is relatively easy, since they were invented with such utilities in mind. Quantum invariants like the Jones polynomial and its generalizations, on the other hand, were discovered in settings removed from topology proper. As such, they are not intrinsically geometric, nor is it often clear how to apply them or even what they \emph{mean.}

It's not surprising, then, that concerted efforts to better understand quantum invariants have come from a variety of directions, including operator algebras, graph theory and combinatorics, perturbation theory, and quantum group representation theory. Witten's work with Feynman path integrals and topological quantum field theories (TQFT) \cite{Witt94_MR1338609} provided some geometric backdrop for the Jones polynomial, but his results were not mathematically rigorous and could provide only philosophical explanations. The Kontsevich integral \cite{Kont94_MR1341841} gives a highly geometric definition of quantum invariants, but is unfortunately very difficult to compute. Until recently, similar attempts have failed to bear significant fruit.

However, quantum topology was revolutionized in 2000 by Mikhail Khovanov. His original theory \cite{Khov00_MR1740682} was a ``categorification" of the Jones polynomial $V(L)$ (the link invariant associated to $\mathfrak{g}=\su{2}$), so described because it associates to any link $L$ a complex $Kh^{i,j}(L)$ of bigraded modules whose graded Euler characteristic is $V(L)$. Not only is the homotopy type of $Kh^{i,j}(L)$ a link invariant, but it contains geometric information about cobordisms into and out of $L$ (ie, knotted surfaces in 4-space) that appears nowhere in $V(L)$ itself.

This versatility quickly led to new geometric results, the first of which was discovered by Jacob Rasmussen \cite{Rasm:SliceGenus}. Given a knot $K$, he uses the algebraic structure of Khovanov homology to define an integer $s(K)$ that gives a lower bound on the \emph{smooth} slice genus of $K$. (In fact, his invariant is sharp for alternating knots.) In the same short paper he gives a purely combinatorial proof of the Milnor Conjecture (specifying the slice genus of a torus knot), which prior to Rasmussen's previous work on Oszvath-Szabo homology had only been proven using gauge theory.

Indeed, it was a wonderful surprise that information about smooth four-dimensional topology could be derived from such an algebraic construction. The hope now is that a great deal more geometric information can be extracted from the algebraic structure of Khovanov's homology theory and its various incarnations. With this goal in mind, we shall now focus on a particular variation of Khovanov homology: the case in which $\mathfrak{g} = \su{3}$.


%
%
%The idea behind Khovanov's original homology construction is relatively simple. In \cite{MR1740682}, he describes a combinatorial recipe for assigning, to any oriented link diagram $D$, a bigraded chain complex $C^{i,j}(D)$ of modules over $\Z$. He then demonstrates that if two diagrams $D$ and $D'$ differ by a single Reidemeister move, there is a canonical homotopy equivalence $C^{i,j}(D) \rightarrow C^{i,j}(D')$ between their complexes. As such, taking the homology of this complex gives a link invariant $Kh^{i,j}(L) := H^{i,j}(C(D))$ for any diagram $D$ of $L$. This construction relies heavily on the Kauffman bracket skein relations (and a writhe correction), a straightforward consequence of which is that, as mentioned earlier, the graded Euler characteristic $\chi Kh^{i,j}(L) = V(L)$.
%
%The novel geometric power of Khovanov's theory, however, comes from its ability to detect cobordism information. A \emph{link cobordism} between two links $L_0$ and $L_1$ in $\R^3$ is an embedded (and possibly knotted) surface $S$ in $\R^{3} \times I$ such that $\partial S = L_0 \amalg L_1$. By virtue of the Frobenius algebra at work in the definition of $C^{i,j}(D)$, Khovanov's construction naturally associates, to any link cobordism $S$, a module homomorphism on homology $$Kh(S): Kh^{\bullet,\bullet}(L_0) \rightarrow Kh^{\bullet,\bullet}(L_1).$$ It was the algebraic structure of this (graded) map that Rasmussen used to define his $s$-invariant, which has since been generalized \cite{Lobb:SliceGenus_sl(n)}.
%
%Taking a step back, though, we see a much more appealing picture. In particular, we observe that Khovanov homology seems to behave like a \emph{functor}: it acts not only on objects (oriented tangles in 3-space) but on morphisms as well (tangles cobordisms in 4-space). Let's call our source category \textbf{Ortang}.
%
%\begin{quest}
%\label{quest:su2funct}
%Is $Kh:$ \emph{\textbf{OrLinkCob}} $\rightarrow \Z$\emph{\textbf{-Mod}} really a functor?
%\end{quest}
%
%This question has far-reaching implications. On the largest scale, it determines whether Khovanov homology acts like a TQFT, and thus whether it may be possible to extend it to three- and four-manifolds. Furthermore, an answer in the negative complicates the maps in Khovanov homology, but may also indicate that the theory can detect extra geometric structure in knotted surfaces.
%
%As it turns out, the answer to Question \ref{quest:su2funct} is ``No": while $Kh$ is clearly well-defined on links, this is not quite the case for cobordisms (which we consider up to isotopy in four-space). In \cite{MR2113903}, Jacobsson shows that the maps $Kh(S)$ are only well-defined up to an overall sign, and actually demonstrates the particular isotopies of $S$ that introduce this ``sign anomaly." The next natural (two-part) question is
%
%\begin{quest}
%\label{quest:su2fix}
%Is it possible to alter Khovanov's theory to make it functorial on \emph{\textbf{LinkCob}}?
%\end{quest}
%
%An idea for an alteration to the original theory came from Scott Morrison and Kevin Walker. There was already significant evidence that orientations somehow needed to play a deeper role, recalling that Khovanov's original theory is built on the \emph{unoriented} skein relations of the Kauffman bracket. Indeed, a convenient set of \emph{piecewise-oriented} (or ``disoriented") skein relations for the Jones polynomial can be derived from the representation theory of $U_q(\mathfrak{sl_2})$. Of key interest is that the fundamental representation of this quantum group is \emph{anti-symmetrically} self-dual. This fact can be hidden when dealing with closed links, but necessitates an additional anti-symmetric skein relation for tangles (embeddings of disjoint arcs in the three-ball).
%
%Inspired by Bar-Natan's construction of a universal Khovanov theory for unoriented tangles in \cite{MR2174270} (in which we must work over the ring $\Z[\frac{1}{2}]$), Morrison and Walker invented a corresponding theory for oriented tangles, built on these disoriented skein relations. They conjectured that this modified theory, $\widetilde{Kh}$, gave the desired functorial behavior. Jointly with Morrison and Walker in \cite{Fix}, I proved this conjecture.
%
%\begin{thm}
%\label{thm:su2f}
%$\widetilde{Kh}$ is an invariant of oriented links. Furthermore, $\widetilde{Kh}:$ \emph{\textbf{OrLinkCob}} $\rightarrow \Z[\frac{1}{2}]$\emph{\textbf{-Mod}} is a functor.
%\end{thm}
%
%

